Data Curation Alone Can Stabilize In-context Learning

In-context learning (ICL) enables large language models (LLMs) to perform new tasks by prompting them with a sequence of training examples. However, it is known that ICL is very sensitive to the choice of training examples: randomly sampling examples from a training set leads to high variance in performance. In this paper, we show that carefully curating a subset of training data greatly stabilizes ICL performance without any other changes to the ICL algorithm (e.g., prompt retrieval or calibration). We introduce two methods to choose training subsets -- both score training examples individually, then select the highest-scoring ones. CondAcc scores a training example by its average dev-set ICL accuracy when combined with random training examples, while Datamodels learns linear regressors that estimate how the presence of each training example influences LLM outputs. Across five tasks and two LLMs, sampling from stable subsets selected by CondAcc and Datamodels improves average accuracy over sampling from the entire training set by 7.7% and 6.3%, respectively. Surprisingly, the stable subset examples are not especially diverse in content or low in perplexity, in contrast with other work suggesting that diversity and perplexity are important when prompting LLMs.

==> Figs/datamodel_w.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=0.85\linewidth]{Figs/ag_news-gpt-j-6b-DatamodelW.pdf}
\caption{Visualizing the \emph{good} training examples selected by \Simple\ and \Datamodels\ in datamodels embedding space. Each dot is a training example in AGNews, where datamodels spontaneously learn to encode class information in the embeddings. Both methods choose tightly clustered sets
of examples, showing \emph{good} subsets are not diverse in the embedding space.}
\label{fig:datamodel_embed}
\end{figure}

==> Figs/divI_divF.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.85\linewidth]{Figs/div-I-div-F.pdf}
\caption{Comparing the diversity of the \emph{good} subset (blue), \emph{bad} subset (red), and randomly smapled subsets (boxplot) on different tasks using GPTJ. Left: diversity in the textual form (DIV-I). Right: diversity in the SentBERT feature space (DIV-F). For both metrics, a higher number means a subset is more diverse. Our \emph{good} subsets are no more diverse than random subsets under both metrics.}
\label{fig:divI_divF}
\end{figure*}

==> tables/retrieval.tex <==
\begin{table*}[!t]
\begin{center}
\centering
%\resizebox{2.0\columnwidth}{!}
{
\begin{tabular}{lcccccc}
\toprule
      & \textbf{SST-2} & \textbf{BoolQ} & \textbf{Subj} & \textbf{Scicite} & \textbf{AGNews} & Avg. Tasks \\

\midrule
\emph{kNN}\\
~ \Sbert & $83.4$ & $52.9$ & $88.4$ & $51.6$ & $77.6$ & $70.8$\\
~ \Roberta & $61.3$ & $54.1$ & $86.1$ & $51.5$ & $59.6$ & $62.5$\\

\midrule
\emph{GPTJ-6B}\\
~ \Sbert & $88.6$ & $63.8$ & $78.2$ & $49.8$ & $82.0$ & $72.5$\\
~ \Roberta & $81.3$ & $64.1$ & $73.0$ & $46.9$ & $75.2$ & $70.3$\\

\midrule
\emph{OPT-13B}\\
~ \Sbert & $85.6$ & $66.3$ & $81.1$ & $47.3$ & $83.9$ & $72.8$\\
~ \Roberta & $73.9$ & $66.7$ & $78.2$ & $45.6$ & $74.7$ & $70.3$\\


\bottomrule
\end{tabular}}
\end{center}

\caption{Results of the instance-dependent prompt retrieval method. We use SentBERT and RoBERTA-large as the sentence encoders. For each test input, we retrieve the most similar training examples in the sentence embedding spaces as the prompt. We also report the $k$NN baseline results ($k=5$) before running in-context learning on GPTJ-6B and OPT-13B.}
\label{table:retrieval}
\end{table*}
